Computing Teichm\"{u}ller Maps between Polygons

By the Riemann-mapping theorem, one can bijectively map the interior of an $n$-gon $P$ to that of another $n$-gon $Q$ conformally. However, (the boundary extension of) this mapping need not necessarily map the vertices of $P$ to those $Q$. In this case, one wants to find the ``best" mapping between these polygons, i.e., one that minimizes the maximum angle distortion (the dilatation) over \textit{all} points in $P$. From complex analysis such maps are known to exist and are unique. They are called extremal quasiconformal maps, or Teichm\"{u}ller maps. Although there are many efficient ways to compute or approximate conformal maps, there is currently no such algorithm for extremal quasiconformal maps. This paper studies the problem of computing extremal quasiconformal maps both in the continuous and discrete settings. We provide the first constructive method to obtain the extremal quasiconformal map in the continuous setting. Our construction is via an iterative procedure that is proven to converge quickly to the unique extremal map. To get to within $\epsilon$ of the dilatation of the extremal map, our method uses $O(1/\epsilon^{4})$ iterations. Every step of the iteration involves convex optimization and solving differential equations, and guarantees a decrease in the dilatation. Our method uses a reduction of the polygon mapping problem to that of the punctured sphere problem, thus solving a more general problem. We also discretize our procedure. We provide evidence for the fact that the discrete procedure closely follows the continuous construction and is therefore expected to converge quickly to a good approximation of the extremal quasiconformal map.

==> approximation.tex <==
\subsection{Approximation guarantee/Discussions}
\label{approximation}

Our discrete algorithm is an analog of the continuous construction; since the continuous construction was proven to converge, it is reasonable to hope that the discrete method will be a good approximation of the exact answer, given a sufficiently dense set and a good triangulation. Solving a Beltrami equation is similar to solving an elliptic PDE, and from the theory of finite elements, assuming a bound on the angles of the triangulation, the solution is within $O(\epsilon^{2})$, where $\epsilon$ is the maximum edge length in the triangulation. We hope to pursue this direction in the future to figure out the factor involved (if any) in our method.



==> squish-macros.tex <==
% !TEX root =  do-all.tex

%%%%%%%%%%%%%%%%%%%%  FOR COMMENTS  %%%%%%%%%%%%%%%%%%%%%%%

% allow toggle between full and short:

%\newcommand{\full}[1]{\#{\bf #1}\# }  %%leave for combined version
\newcommand{\full}[1]{}               %%leave for short version
%\newcommand{\full}[1]{#1}              %%leave for full version

%\newcommand{\short}[1]{\${\em #1}\$ } %%leave for combined version
\newcommand{\short}[1]{#1}            %%leave for short version
%\newcommand{\short}[1]{}               %%leave for full version

% named comments:
%\newcommand{\estie}[1]{\textbf{Estie:} #1}
%\newcommand{\michael}[1]{\textbf{Michael:} #1}
%\newcommand{\joe}[1]{\textbf{Joe:} #1}

% to blank out text:
\newcommand{\old}[1]{{}}

\newcommand{\comm}[1]{{\em COMMENT: #1}}

% margin comments:
% \newcommand{\comment}[1]{\marginpar{{\footnotesize #1}}}

%%%%%%%%%%%%%% SOME ABBREVIATIONS AND NOTATIONS %%%%%%%%%%%%%%

\newcommand{\eps}{\varepsilon}               % epsilon

\def\A{{\cal A}}
\def\B{{\cal B}}
\def\C{{\cal C}}
\def\D{{\cal D}}
\def\E{{\cal E}}
\def\F{{\cal F}}
\def\G{{\cal G}}
\def\H{{\cal H}}
\def\I{{\cal I}}
\def\J{{\cal J}}
\def\K{{\cal K}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\N{{\cal N}}
\def\O{{\cal O}}
\def\P{{\cal P}}
\def\Q{{\cal Q}}
\def\R{{\cal R}}
\def\S{{\cal S}}
\def\T{{\cal T}}
\def\U{{\cal U}}
\def\V{{\cal V}}
\def\W{{\cal W}}
\def\X{{\cal X}}
\def\Y{{\cal Y}}
\def\Z{{\cal Z}}

%%%%%%%%%%%%%%%%%%%%%% SQUISHTEX  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Very flexible definitions of \section, \subsection, \subsubsection, and
% \paragraph.  The lengths \above[sub[sub]]sectionskip, \aboveparagraphskip,
% \below[sub[sub]]sectionskip, and \belowparagraphskip control the space around
% the headings.  If the below skips are negative, the section title is on the
% same line as the next paragraph.  The commands \[sub[sub]]sectionfont and
% \paragraphfont define the fonts for the headings.  By default, they produce
% the same effect as the article document class.
\newlength\abovesectionskip
\abovesectionskip=3.5ex plus .2ex minus 1ex
\newlength\belowsectionskip
\belowsectionskip=2.3ex plus .2ex
\def\sectionfont{\normalfont\Large\bfseries}
\newlength\abovesubsectionskip
\abovesubsectionskip=3.25ex plus .2ex minus 1ex
\newlength\belowsubsectionskip
\belowsubsectionskip=1.5ex plus .2ex
\def\subsectionfont{\normalfont\large\bfseries}
\newlength\abovesubsubsectionskip
\abovesubsubsectionskip=3.25ex plus .2ex minus 1ex
\newlength\belowsubsubsectionskip
\belowsubsubsectionskip=1.5ex plus .2ex
\def\subsubsectionfont{\normalfont\normalsize\bfseries}
\newlength\aboveparagraphskip
\aboveparagraphskip=-3.25ex plus 1ex minus .2ex
\newlength\belowparagraphskip
\belowparagraphskip=-1em
\def\paragraphfont{\normalfont\normalsize\bfseries}
\makeatletter
\def\section{\@startsection{section}{1}{\z@}{-\abovesectionskip}%
              {\belowsectionskip}{\sectionfont}}
\def\subsection{\@startsection{subsection}{1}{\z@}{-\abovesubsectionskip}%
                 {\belowsubsectionskip}{\subsectionfont}}
\def\subsubsection{\@startsection{subsubsection}{1}{\z@}%
                    {-\abovesubsubsectionskip}{\belowsubsubsectionskip}%
                    {\subsubsectionfont}}
\def\paragraph{\@startsection{paragraph}{4}{\z@}{-\aboveparagraphskip}%
                {\belowparagraphskip}{\paragraphfont}}
\makeatother

% Here are some good tight spacings for sections.
\abovesectionskip=1ex plus .5ex minus .5ex
\belowsectionskip=.5ex plus .5ex minus .25ex
\abovesubsectionskip=.75ex plus .75ex minus .375ex
%\abovesubsectionskip=.5ex plus .5ex minus .25ex
\belowsubsectionskip=.5ex plus .5ex minus .25ex
\aboveparagraphskip=.5ex plus .5ex minus .25ex
%\aboveparagraphskip=.25ex plus .25ex minus .125ex
\abovesubsubsectionskip=.5ex plus .5ex minus .25ex
\belowsubsubsectionskip=-1em

% Times font is thinner and saves space
\usepackage{times}

% Decrease space around theorems and such
\partopsep=3pt
\parsep=0pt
\topsep=0pt

% Reduce the extra space caused by displaymath (\[ ... \])
\abovedisplayskip=2pt plus 1pt minus 1pt
\belowdisplayskip=2pt plus 1pt minus 1pt
\abovedisplayshortskip=1pt plus 1pt minus 1pt
\belowdisplayshortskip=1pt plus 1pt minus 1pt

% Figure spacing
\abovecaptionskip=0pt           % space between figure and caption
\belowcaptionskip=0pt           % space after caption except for bottom figure
\intextsep=7pt plus 3pt        % space between [h]ere figure and text
\textfloatsep=7pt plus 3pt     % space between [t]op or [b]ottom figure & text

% Compact itemize and enumerate.  Note that they use the same counters and
% symbols as the usual itemize and enumerate environments.
\def\compactify{\itemsep=0pt \topsep=0pt \partopsep=0pt \parsep=0pt}
\let\latexusecounter=\usecounter
\newenvironment{CompactItemize}
 {\def\usecounter{\compactify\latexusecounter}
  \begin{itemize}}
 {\end{itemize}\let\usecounter=\latexusecounter}
\newenvironment{CompactEnumerate}
 {\def\usecounter{\compactify\latexusecounter}
  \begin{enumerate}}
 {\end{enumerate}\let\usecounter=\latexusecounter}


%%%%%%%%%%%%%%%%%%%%%%% END SQUISH




==> vectorfield.tex <==
\subsection{Vector field method}
\label{subsec:vectorfield}
For brevity let $\alpha = (\mu_{h} - \upsilon_{h})$. Note that $\alpha$ is infinitesimally trivial. In this section we will describe a method to get the curve $\mu_{g}(t) = t\alpha + O(t^{2})$ which satisfies the hypothesis of Lemma \ref{reductionlemma}. The Mapping Theorem, which we state in the appendix \ref{mapping}, is important for the analysis of our construction.

Observe that as a consequence of the fact that $\alpha$ is infinitesimally trivial, the mapping theorem implies that \textit{the image of $z_{i}$ under $f^{t \alpha}$ is within $O(t^{2})$  of $z_{i}$}. Note that $0,1$ and $\infty$ are fixed. Let $f^{t \alpha}(z_{i}) = {z_{i}}^{'}$.

We will first construct self homomorphisms $p_{t}$ of the sphere such that $p_{t}(z_{i}^{'})={z_{i}}$ and $||\mu_{p_{t}}||_{\infty} = O(t^{2})$. Once this is done, we define $g_{t} =  p_{t} \circ f^{t \alpha}$. Then by the formula for composition \ref{formula}, one concludes that $\hat{\mu}_{g}(t) = t \alpha + O (t^{2})$, which is what was desired in the hypothesis of Lemma \ref{reductionlemma}.

To construct $p_{t}$, let
\[\displaystyle\max_{1\leq i \leq n-3} |z_{i}| = r\] Applying the Mapping Theorem \ref{mapping} we get,

\begin{equation}\label{closeness}
|z_{i}^{'} - z_{i}| < C_{r} t^{2}
\end{equation}


where $C_{r}$ is a constant depending only on $r$. Let $d_{i} = |z_{i}-z_{i}^{'}|$ and $\displaystyle\min_{i,j} |z_{i}-z_{j}| = d$. For $t$ sufficiently small, we can assume that $C_{r}t^{2} < d/4$. Let $B_{r}(z)$ denote the open disk of radius $r$ centered at $z$. It is clear that the disks $\{B_{d/2}(z_{i}^{'})\}_{i=1}^{n-3}$ are disjoint  and ${z_{i}} \in B_{d/2}(z_{i}^{'})$.
The idea is to design a vector field with support on $\cup_{i} B_{d/2}(z_{i}^{'})$ such that the integral curve of this vector field sends $z_{i}$ to $z_{i}^{'}$. We show how to design this vector field on one particular disk $B_{d/2}(z_{i})$.
By applying a rotation, we can assume that the line segment $z_{i}^{'}z_{i}$ is aligned with the positive x-axis. Pick a $C^{\infty}$ function $f_{i}$ such that
\begin{enumerate}
\item $f_{i}(z) = 0$ for $z \in \mathbb{C} \setminus B_{d/2}(z_{i}^{'})$.
\item $f_{i}(z)=d_{i}$ for $z \in B_{2d_{i}}(z_{i}^{'})$.
\end{enumerate}
Consider the vector field
\[ V_{i}(z) = f_{i}(z) \frac{\partial}{\partial x} \]

Clearly, the integral curve for this field for unit time will send $z_{i}$ to $z_{i}^{'}$. This self diffeomorphism of $B_{d/2}(z_{i})$ introduces no dilatation where $f_{i}$ equals 1, since locally the map is a translation. Note that the vector fields $\{V_{i}\}_{i=1}^{n-3}$ piece up together to get one vector field on $\hat{\mathbb{C}}$. All that needs to be shown is that the Beltrami coefficent of this self map is $O(t^{2})$:

The trick is to choose the cut-off function on a fixed small neighborhood of each point, such that the definition of the cut-off function does not involve $t$. We will let $s$ denote the parameter for the one-parameter family of diffeomorphisms $\gamma$ associated with our vector field. Let $r_{t}$ be the trajectory of the point $z_{i}$, and let $p$ be the cutoff function. Then the vector field is given by 

\begin{equation}
X_{t} = p (\gamma_{t})(z^{'} - z)
\end{equation}

Now, $X_{t} = \frac{\partial \gamma_{t}}{\partial s}$. Differentiation w.r.t $z$ gives
\begin{equation}
\frac{\partial (\gamma_{t})^{'}}{\partial s} = \left( \frac{\partial p}{\partial z} \gamma^{'}(t) + \frac{\partial p}{\partial \bar{z}}  {\overline{\gamma}}^{'}(t) \right) (z^{'} - z)
\end{equation}

Since $|z^{'} - z| = O(t^{2})$ by the Mapping Theorem \ref{mapping}, evaluating the derivative of the above equation at $t=0$ gives


\begin{equation}
\frac{\partial (\gamma_{t})^{'}}{\partial s}||_{t=0} = 0
\end{equation}
This means that $\gamma_{t}^{'}(t=0)$ is constant in $s$, implying that $\gamma_{t}^{'} (t=0,s) = \gamma_{t}^{'} (t=0,s=0) = 0$. Now $\gamma_{t} = id$ when $s=0$. Similarly we get the derivative w.r.t $\bar{z}$ as $0$.

The beltrami coefficient $\mu_{t} = \frac{\gamma_{t,\bar{z}}}{\gamma_{t,z}}$. We evaluate the derivative w.r.t. and put $t=0$ to get


\begin{equation}
\frac{((\gamma_{t \bar{z}}^{'}(0))\gamma_{0z} ) - ((\gamma_{tz}^{'}(0))\gamma_{0z})}{(\gamma_{0z}^{2})}
\end{equation}

which by the above findings is $0$. Hence there is no $O(t)$ term and we are done.


